Inference-Based Deterministic Messaging For Multi-Agent Communication

Communication is essential for coordination among humans and animals. Therefore, with the introduction of intelligent agents into the world, agent-to-agent and agent-to-human communication becomes necessary. In this paper, we first study learning in matrix-based signaling games to empirically show that decentralized methods can converge to a suboptimal policy. We then propose a modification to the messaging policy, in which the sender deterministically chooses the best message that helps the receiver to infer the sender's observation. Using this modification, we see, empirically, that the agents converge to the optimal policy in nearly all the runs. We then apply this method to a partially observable gridworld environment which requires cooperation between two agents and show that, with appropriate approximation methods, the proposed sender modification can enhance existing decentralized training methods for more complex domains as well.

==> source/old_experiments.tex <==
% old experiments section
% obsolete now, but contains some useful comments (I will add back to new section 4.1)

\label{section:experiments}

\subsection{Environment}

%\begin{floatingfigure}[r]{0.35\textwidth}
\begin{wrapfigure}{r}{0.33\linewidth}
%\begin{figure}[b]
  \centering
  \vspace{-1cm}
  \includegraphics[width=0.3\columnwidth]{images/climbing_game.pdf}
  \caption{Payoffs for the climbing game.}
  \label{fig:climbing_game}
%\end{figure}
%\end{floatingfigure}
\end{wrapfigure}
In our experiments, we consider the games defined in Section~\ref{sec:intro}.
One set has three states, three messages and three actions, and the other set
has 32 states, messages and actions. We use payoffs shown in
Figure~\ref{fig:climbing_game} to explain the issue of convergence to a
sub-optimal policy. This payoff matrix is a normalized version of climbing
game~\cite{claus1998dynamics} that is used in MARL literature to study
learning algorithms for simultaneous action games.
%%%mic: redundant: Henceforth, we will be referring to the payoff matrix shown in the figure when we say `the climbing game'.
We then perform experiments on a set of 1,000 payoff matrices each of sizes
3x3 and 32x32, with each payoff generated uniformly randomly between 0 and 1
and normalized such that the maximum payoff is 1, to show that this issue is
not specific to the climbing game.

\subsection{Training Method}

Each run of our experiments lasted for 1,000 episodes in case of a 3x3 payoff
matrix and 25,000 episodes in case of a 32x32 payoff matrix. In each episode, first
a uniform random state was generated and passed to the sender. The sender then
computed its message and sent it to the receiver, which used the message to
compute its action. Finally, the reward corresponding to the state and the
action was then sent to both agents. The obtained rewards (normalized by the
maximum reward) and the converged policies of the agents were recorded.

For each algorithm and each payoff matrix, this process was repeated 1,000 times.
The mean of the normalized obtained rewards and percentage of the runs which
converged to the optimal policy were recorded. This whole process was then
repeated for all 1,000 payoff matrices, recording the mean of the normalized
rewards and percentage of optimal convergence over all payoff matrices.

%%%% 
We performed hyper-parameter tuning using a combination of grid search and
manual tuning. We generated 100 random payoff matrices, and for each set of
hyper-parameters and each payoff matrix, we ran 1,000 runs as described
above. The set of hyper-parameters with the highest percentage of runs that
converged to optimal policy was used in all other experiments.
Hyper-parameter tuning was performed separately for 3x3 payoff matrices and
32x32 payoff matrices.

The experiments with payoffs similar to the climbing game were also performed
in the same fashion, with 1,000 runs for each algorithm, as described in the
first paragraph.

\subsection{Considered Benchmark Algorithms}

In what follows, we compare our new method with variants of traditional
single-agent RL algorithms and algorithms from the literature that have been
shown to be effective in cooperative games with simultaneous actions.
%
Here, we only briefly describe the algorithms. More detailed descriptions
including parameter choices can be found in Appendix~\ref{appendix:algorithms}.
%
For our experiments we consider:

$\bullet$ \textbf{Info-Q} -- The algorithm with information maximizing sender
proposed in this paper. The sender uses Algorithm~\ref{alg:sender} and the
receiver uses Algorithm~\ref{alg:receiver} modified to select actions greedily
since we found that $\epsilon$-greedy exploration by the receiver was not
required for the experimental domains that we chose in this paper.

$\bullet$ \textbf{Info-Policy} -- Similar to Info-Q, but the receiver uses a
policy gradient method (REINFORCE) instead of Q-Learning.

$\bullet$ \textbf{Fixed messages or fixed actions} -- For each algorithm, we
ran a version in which the policy of either the sender or the receiver was
fixed to an optimal one and only the other agent is trained. With this, the
problem was reduced to a single-agent problem. Therefore, we excluded these
results in the comparison. \comm{why mention them here then? They don't seem
  to be mentioned in the text, either. Nevertheless, can their results be
  added - as some kind of a lower bound?}

$\bullet$ \textbf{Independent Q-Learning (IQL)} -- Both the sender and the
receiver are trained independently using Q-Learning. The sender maintains a
Q-table with entries for each state and each message, while the receiver
maintains entries for each message and each action.

$\bullet$ \textbf{Iterative Learning (IQ)} -- The learning is iterative, with
the sender updating its policy for a certain number of episodes, while the
receiver is fixed, followed by the receiver updating its policy while the
sender is fixed, and so on.

$\bullet$ \textbf{Model the sender (Model1 \comm{ModelS seems more
    intuitive})} -- The receiver maintains a Q-table for each state and each
action, in addition to a Q-table for each state and each message to model the
sender. \comm{need more details here?}

$\bullet$ \textbf{Model the receiver (Model2 \comm{ModelR seems more
    intuitive})} -- The sender maintains a Q-table for each state and each
action. It also maintains a Q-table for each message and each action to model
the receiver. \comm{need more details here?}

$\bullet$ \textbf{Hysteretic-Q} -- An adaptation of the algorithm given by
\citet{matignon2007hysteretic} to our problems. The idea is to use a higher
step size for positive updates and a lower step size for negative
updates. \comm{explain what positive and negative updates are, what is
  sender/receiver learning based on? Add more details to appendix as
  well}

$\bullet$ \textbf{Lenience} -- An adaptation of the algorithm presented in
\citet{panait2006lenience} (specifically the RL version given by
\citet{wei2016lenient}). In the initial time steps, Q-values are updated only
if the update is positive, ignoring low rewards. As the number of episodes
increases, Q-values are always updated. \comm{explain what sender/receiver is
  based on. Add more details to appendix as well}


==> source/problem.tex <==
In this paper we consider the problem of learning to communicate
%%%mic: was: with
through a no-cost channel
%%%mic: repeat: (also known as cheap-talk channel)
in cooperative games with independent 
learners. Formally, there are
two agents, a sender and a receiver. At each time step, the sender gets a state
$s$, based on which it sends a message $m$ to the receiver. The receiver
observes the message (but not the state) and takes an action $a$. Then, both the
agents receive
%%%mic: removed "a"
reward $r=R(s,a)$ that is not affected by the
%%%mic: was: message shared.
sent message.

The receiver
%%%mic: was: does not
cannot observe state $s$ during execution and training. The sender
%%%mic: was: does not
cannot observe action $a$ taken by receiver and, hence, cannot use it during
training. These restrictions are relaxed for some of the
%%%mic: was: baselines
baseline algorithms for which $s$ and $a$ are available to both agents during
training.
%%%mic: was: Additionally, the training algorithms should be decentralized,
Lastly, we only consider decentralized training algorithms in which each agent
maintains its own parameters and updates them only dependent on the
information it observes. \comm{add motivation why we insist on decentralized
learning?}


==> source/results.tex <==
\subsection{Learning Results for the Climbing Game}

Experiments with the climbing game are performed using the payoff matrix 
given in Figure~\ref{fig:climbing_game} to highlight the issues with the 
existing algorithms.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/norm_reward_climbing.pdf}
    \caption{Normalized reward obtained during training, as a function of
    episodes for the climbing game. Standard error across the runs is less than
    the line width. Info-Q converged to an optimal policy in around 300
    episodes.}
    \label{fig:norm_reward_climbing}
%\end{figure}
%
%\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{images/opts.pdf}
    \caption{Percentage of runs that took the optimal actions, as a
    function of episodes for the climbing game. The difference between the
    algorithms is magnified in this plot since the sub-optimal reward may be
    close in value to an optimal payoff.}
    \label{fig:opts}
\end{figure}

Figure~\ref{fig:norm_reward_climbing} shows the plot of the mean normalized
reward, as a function of episodes. Figure~\ref{fig:opts} shows the percentage of
runs that took the optimal actions, as a function of episodes. While
some of the algorithms obtain rewards close to that obtained by Info-Q, the
difference is magnified in the plot of percentage of runs that converge to an
optimal policy.

%%%mic: (state, action)-pairs better than "state, action pairs"
For obtaining more insights into the potential issues of the the baseline
algorithms, we count (state, action)-pairs for each run. We iterate through
the states, and for each state we calculate the corresponding message sent by
the sender and the action taken by the receiver. Figure~\ref{fig:cps} shows
the matrix with the counts for each (state, action)-pair in case of
Independent Q-Learning (IQL, on the left) and Info-Q (on the right). It can be
observed that in state $s_2$ (middle row), the receiver takes action $a_3$
(last column) with Q-Learning, while in case of Info-Q, it takes action $a_2$
(middle column), which is the optimal action.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.8\columnwidth]{images/cp_iql.pdf}
%     \caption{Counts of (state, action)-pairs for IQL. The receiver takes $a_3$ in
%     $s_2$, even though $a_2$ is the optimal action to take.}
%     \label{fig:cp_iql}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.8\columnwidth]{images/cp_infoq.pdf}
%     \caption{Counts of (state, action)-pairs for Info-Q. All runs converge to the
%     optimal policy}
%     \label{fig:cp_infoq}
% \end{figure}

%%%mic: use [t] or [b] to move figures up or down

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{images/cps.pdf}
    \caption{Counts of (state, action)-pairs for IQL and Info-Q for the climbing game.
    With IQL, the receiver took $a_3$ in $s_2$, even though $a_2$ is the optimal
    action to take. With Info-Q, all runs converged to an optimal policy.}
    \label{fig:cps}
%\end{figure}

    \medskip

%\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/venns.pdf}
    \caption{Venn diagram of messaging policy for IQL and Info-Q. Intersections
    in case of IQL imply that in some runs, multiple states were assigned the
    same message. In case of Info-Q, all states were assigned a distinct message.}
    \label{fig:venns}
\end{figure}


We also plot Venn diagrams to visualize the messaging policy. Figure~\ref{fig:venns}
shows the Venn diagrams for independent Q-Learning (on the
left) and Info-Q (on the right). The region labeled $s_i$ outside any
intersection corresponds to runs in which $s_i$ was assigned a unique
%%%mic: a unique (u is pronounced ju - so no vovel ...
message. The intersection of regions $s_i$ and $s_j$ denote the runs in which
$s_i$ and $s_j$ were assigned the same message. The intersection of all
regions corresponds to runs in which all states were assigned the same
message. Info-Q assigns a distinct message to each state, whereas there are
some Q-Learning runs that assign the same message to multiple states.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{images/venn_iql.pdf}
%     \caption{Venn diagram of messaging policy for IQL. Intersections imply that
%     in some runs, multiple states were assigned the same message.}
%     \label{fig:venn_iql}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{images/venn_infoq.pdf}
%     \caption{Venn diagram of messaging policy for Info-Q. All states are
%     assigned a distinct message.}
%     \label{fig:venn_infoq}
% \end{figure}

The combination of (state, action)-pair counts and the Venn diagrams suggest
that Q-Learning is converging to a sub-optimal policy of choosing $a_3$
in $s_2$. We hypothesize that this is due to the closeness of the two payoffs
and the fact that $a_3$ is a `safer' action to take since the penalty is not
very high if the message was incorrect. The messages corresponding to $s_2$
and $s_3$ are the same in many runs. A possible reason for this is that, since
the receiver is more likely to take $a_3$, there is insufficient incentive to
send a separate message for $s_2$ and $s_3$. We believe that this vicious
cycle leads to the agents converging to a sub-optimal policy. Info-Q
overcomes this cycle by forcing the sender to fully utilize the communication
channel irrespective of the incentive it receives through the rewards.

\subsection{Learning Results for Random Payoff Games}

To ensure that the issues were not specific to a single game, we generated random 
payoff matrices of size 3x3 and 32x32, and performed experiments using them.

Figures~\ref{fig:norm_reward},~\ref{fig:norm_reward_32x32} show the plots of the mean
normalized reward, as a function of episodes, on 3x3 and 32x32 payoff matrices respectively.
The mean, here, refers to all random payoff matrices and
multiple runs for each payoff matrix. Figures~\ref{fig:boxplot},~\ref{fig:boxplot_32x32} show the
boxplots (between 25 and 75 percentile) of the percentage of runs that converge
to an optimal policy
for each payoff matrix of size 3x3 and 32x32 respectively. The boxplots clearly show the difference between
Info-Q and the other algorithm in terms of convergence to an optimal
policy. 
%\comm{again, to ... an optimal policy?}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/norm_reward.pdf}
    \caption{Mean normalized reward obtained during training, as a function of episodes, on random 3x3 payoff matrices.
    %\comm{is this test reward (i.e., exploration switched off?}
    %%%reply: No. It is the reward obtained during training
    One standard error is shaded
    % \comm{hard to see}
    %%%reply: The standard error is very low, so it is merged with the line width in many cases
    , but it is less than the line width in most cases. Info-Q obtained the
    maximum reward in almost every state after around 400 episodes.}
    \label{fig:norm_reward}
%\end{figure}
%
%\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{images/boxplot.pdf}
    \caption{Boxplot (between 25 and 75 percentile) of the percentage of runs
    that converged to an optimal policy for each 3x3 payoff matrix.
      %\comm{adding the regret curves is helpful, too}
      %%%reply: There is not enough space to fit it
      Info-Q converged to an optimal policy in nearly all
      runs for all payoff matrices.}
    \label{fig:boxplot}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/norm_reward_32x32.pdf}
    \caption{Mean normalized reward obtained during training, as a function of episodes, on random 32x32 payoff matrices.
    One standard error is shaded, but it is less than the line width in most cases.
    Info-Q obtained the maximum reward in almost every state after around 20000 episodes.}
    \label{fig:norm_reward_32x32}
%\end{figure}
%
%\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{images/boxplot_32x32.pdf}
    \caption{Boxplot (between 25 and 75 percentile) of the percentage of runs
    that converged to an optimal policy for each 32x32 payoff matrix.
      %\comm{adding the regret curves is helpful, too}
      %%%reply: There is not enough space to fit it
      Info-Q converged to an optimal policy in nearly all
      runs for all payoff matrices.}
    \label{fig:boxplot_32x32}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\columnwidth]{images/hard_payoffs_1.pdf}

    \includegraphics[width=0.5\columnwidth]{images/hard_payoffs_2.pdf}

    \includegraphics[width=0.5\columnwidth]{images/hard_payoffs_3.pdf}
    \caption{Three payoff matrices among the randomly generated ones that
    resulted in lowest percent convergence to optimal policy (taken as a
    mean over all algorithms). A common theme among these is that an optimal
    action for a state has a payoff close to that of another action for the same
    state, and the sub-optimal action has higher payoff in other states compared
    to an optimal action.}
    \label{fig:hard_payoffs}
\end{figure}

The version of our algorithm with the receiver being trained using policy
gradient (Info-Policy) does not perform as well as Info-Q. This is due to
policy gradient method itself being slower to learn in this problem (other
algorithms are value-based). IQ works
fairly well in many problems since it is approximately equivalent to iterative
best response. It fails in cases in which iterative best response converges to
a sub-optimal policy. Since the agents explore more at the beginning of a period,
the obtained reward is much lower. Hence, the reward curve for IQ does not truly
reflect its test-time performance. Modelling the sender only works well if the state is known to the
receiver in hindsight (but still not as good as Info-Q). Without knowing the
state in hindsight, the performance is as shown here. Hysteretic-Q converged
to an optimal policy in the case of the climbing game when the number of episodes
was increased from 1,000 to 1e6. It could potentially converge to an optimal 
policy for random payoff matrices too if given enough episodes. But with a lower 
number of episodes, the
percentage of runs with optimal convergence is lower. 
% \comm{this is an
%   additional data point, do you have data for the other algorithms as well?
%   then you could create a log-linear graph telling the reader how things
%   develop when the number of episodes is ridiculous}

Figure~\ref{fig:hard_payoffs} shows examples of some of the randomly generated
3x3 payoff matrices that were hard for the algorithms in terms of convergence to
an optimal policy. The three of the shown ones have the lowest mean
percentage of convergence to an optimal policy across all the
algorithms. Info-Q converges to an optimal policy in all the runs with
these payoff matrices. We hypothesised in the previous subsection that low
percentage of convergence to optimal policy is due to the closeness in
the payoffs of optimal and  sub-optimal actions in a state, combined with
an sub-optimal action having higher payoffs in other states. This hypothesis
is strengthened by these payoff matrices, since they too have the same
issues. Multiple pairs of actions in the top game, $a_1$ and $a_3$ in $s_3$ in
the middle game, and $a_1$ and $a_3$ in $s_2$ in the bottom game have close
payoffs. In each case, the sub-optimal action has a higher expected payoff
across all the states. Further insights into the dynamics of the algorithms
will be required before the hypothesis can be confirmed.

